SARA-RT: Scaling up Robotics Transformers with Self-Adaptive Robust Attention

We present Self-Adaptive Robust Attention for Robotics Transformers (SARA-RT): a new paradigm for addressing the emerging challenge of scaling up Robotics Transformers (RT) for on-robot deployment. SARA-RT relies on the new method of fine-tuning proposed by us, called up-training. It converts pre-trained or already fine-tuned Transformer-based robotic policies of quadratic time complexity (including massive billion-parameter vision-language-action models or VLAs), into their efficient linear-attention counterparts maintaining high quality. We demonstrate the effectiveness of SARA-RT by speeding up: (a) the class of recently introduced RT-2 models, the first VLA robotic policies pre-trained on internet-scale data, as well as (b) Point Cloud Transformer (PCT) robotic policies operating on large point clouds. We complement our results with the rigorous mathematical analysis providing deeper insight into the phenomenon of SARA.

==> action_representation.tex <==
%older variant
\subsubsection{Action representation} 
\label{sec:tokenizer} We experiment with two forms of action representation. Robot actions can be represented by a set of vectors corresponding to positional and rotational displacements, a scalar to track the level of extension of the gripper, and a special vector to represent the command for terminating the episode. Traditionally we would discretize the continuous dimensions (i.e. all except the special one that corresponds to termination of the episode) into 256 bins, and the full robot command would be represented as a sequence of integers (which we denominate \textit{action tokens}). This can be represented as a string of integers, which can then be tokenized as usual by the VLM (for PALI-X, each integer up to 1000 corresponds to a unique token). Alternatively, we can simply describe the actions by the vectors corresponding to displacements/gripper/terminate themselves. To avoid very long sequences, we round the continuous dimensions to 4 decimal places, and represent the action as a string consisting of a sequence of vectors. We call this the \textit{vector representation} of the action space. Again, this string is tokenized as usual into text tokens, and considered as the expected output of PaLI-X. We notice that the vector representation of actions results into higher quality models, with the drawback of outputting longer sequences.  
